Tweak: Towards Portable Deep Learning Models for Domain-Agnostic LoRa Device Authentication

Deep learning based device fingerprinting has emerged as a key method of identifying and authenticating devices solely via their captured RF transmissions. Conventional approaches are not portable to different domains in that if a model is trained on data from one domain, it will not perform well on data from a different but related domain. Examples of such domains include the receiver hardware used for collecting the data, the day/time on which data was captured, and the protocol configuration of devices. This work proposes Tweak, a technique that, using metric learning and a calibration process, enables a model trained with data from one domain to perform well on data from another domain. This process is accomplished with only a small amount of training data from the target domain and without changing the weights of the model, which makes the technique computationally lightweight and thus suitable for resource-limited IoT networks. This work evaluates the effectiveness of Tweak vis-a-vis its ability to identify IoT devices using a testbed of real LoRa-enabled devices under various scenarios. The results of this evaluation show that Tweak is viable and especially useful for networks with limited computational resources and applications with time-sensitive missions.

==> Comments.tex <==
%%% 6/8/22
- add a couple of sentences at the begining of each section (e.g., Sec V.) introducuing the scope of the section

section: experimental setup
- [DONE] DNN section needs to be moved to Results section
- [DONE] exprimental scenarios: put in a table could be better; there is some redundacy with Same Tx, Different Tx etc.

section: results:
- [DONE] did you define what 'vanilla' model is?
- [DONE] caption of subfigure should be done via caption, not adding (a) etc. Did fig 13

NOTES:

I have modified the `closed-set' evaluation sections (hardware, channel, and configuration portability). >>>Let me know if these parts need further work.<<<

I have removed the background section in favor of integrating the background into the 'proposed technique' section. 

I also removed the background information on the hardware impairments...this is because they have been well covered in other works on RF fingerprinting, and my work does not rely on the particular extraction of one kind of impairment (was excessive background for my technique)


I still need to:
- Edit the `open-set' evaluation section (I plan on making this similar to the current `closed-set' section)
- Edit the first few paragraphs of the 'proposedtechnique.tex' section (needs to reflect changes in this section)

